A Logic-Based Framework for Natural Language Inference in Dutch

We present a framework for deriving inference relations between Dutch sentence pairs. The proposed framework relies on logic-based reasoning to produce inspectable proofs leading up to inference labels; its judgements are therefore transparent and formally verifiable. At its core, the system is powered by two ${\lambda}$-calculi, used as syntactic and semantic theories, respectively. Sentences are first converted to syntactic proofs and terms of the linear ${\lambda}$-calculus using a choice of two parsers: an Alpino-based pipeline, and Neural Proof Nets. The syntactic terms are then converted to semantic terms of the simply typed ${\lambda}$-calculus, via a set of hand designed type- and term-level transformations. Pairs of semantic terms are then fed to an automated theorem prover for natural logic which reasons with them while using the lexical relations found in the Open Dutch WordNet. We evaluate the reasoning pipeline on the recently created Dutch natural language inference dataset, and achieve promising results, remaining only within a $1.1-3.2{\%}$ performance margin to strong neural baselines. To the best of our knowledge, the reasoning pipeline is the first logic-based system for Dutch.

==> solved_by_LP.tex <==
% sen_id(109, 168, 'p', 'TEST', 'no', 'Een kind slaat een honkbal').
% sen_id(110, 168, 'h', 'TEST', 'no', 'Een kind mist een honkbal').
% sen_id(111, 175, 'p', 'TEST', 'yes', 'Een familie kijkt naar een kleine jongen die een honkbal raakt').
% sen_id(108, 175, 'h', 'TEST', 'yes', 'Een jongen slaat een honkbal').
% sen_id(111, 177, 'p', 'TEST', 'yes', 'Een familie kijkt naar een kleine jongen die een honkbal raakt').
% sen_id(109, 177, 'h', 'TEST', 'yes', 'Een kind slaat een honkbal').
% sen_id(510, 798, 'p', 'TEST', 'no', 'Twee mensen zitten in de sneeuw zonder kleren, wat zorgt voor camouflage').
% sen_id(507, 798, 'h', 'TEST', 'no', 'Twee mensen zitten in de sneeuw, met kleren aan die voor camouflage zorgen').
% sen_id(566, 897, 'p', 'TEST', 'no', 'Mensen zitten op een strand vol zand bij de oceaan en genieten van een zonnige dag').
% sen_id(565, 897, 'h', 'TEST', 'no', 'Er is niemand aan de wal').
% sen_id(726, 1158, 'p', 'TEST', 'no', 'Een vrouw haalt de ingrediënten uit een kom').
% sen_id(725, 1158, 'h', 'TEST', 'no', 'Een vrouw voegt ingrediënten toe aan een kom').
% sen_id(980, 1556, 'p', 'TEST', 'yes', 'Een man draagt een boom').
% sen_id(981, 1556, 'h', 'TEST', 'yes', 'Een man draagt een plant').
% sen_id(2240, 3606, 'p', 'TEST', 'yes', 'Een aap rijdt op een motor').
% sen_id(2241, 3606, 'h', 'TEST', 'yes', 'Een aap rijdt op een fiets').
% sen_id(2530, 4092, 'p', 'TEST', 'no', 'De persoon tekent niet').
% sen_id(2525, 4092, 'h', 'TEST', 'no', 'Een man tekent een foto').
% sen_id(1970, 4470, 'p', 'TEST', 'yes', 'Een man schopt een voetbal').
% sen_id(2747, 4470, 'h', 'TEST', 'yes', 'Een man schopt een bal').
% sen_id(2983, 4925, 'p', 'TEST', 'yes', 'Iemand doet ingrediënten in een wok').
% sen_id(2984, 4925, 'h', 'TEST', 'yes', 'Iemand doet de ingrediënten in een pan').
% sen_id(3104, 5140, 'p', 'TEST', 'yes', 'Een man heeft plezier met water').
% sen_id(3105, 5140, 'h', 'TEST', 'yes', 'Een man speelt met water').
% sen_id(3833, 6356, 'p', 'TEST', 'no', 'Een vrouw in een rode jurk is een instrument aan het opbergen').
% sen_id(3831, 6356, 'h', 'TEST', 'no', 'Een vrouw in een rode jurk bespeelt een instrument').
% sen_id(4519, 7413, 'p', 'TEST', 'yes', 'Een hond rent achter een bal aan in het gras').
% sen_id(4520, 7413, 'h', 'TEST', 'yes', 'Een hond zit achter een bal aan in het gras').
% sen_id(4845, 7922, 'p', 'TEST', 'yes', 'Een hond rent door een veld en zit achter een bal aan').
% sen_id(4843, 7922, 'h', 'TEST', 'yes', 'Een hond loopt naar een stuk speelgoed toe').
% sen_id(4845, 7924, 'p', 'TEST', 'yes', 'Een hond rent door een veld en zit achter een bal aan').
% sen_id(4842, 7924, 'h', 'TEST', 'yes', 'Een hond loopt naar een bal toe').
% sen_id(5875, 9480, 'p', 'TEST', 'yes', 'Een zwarte hond en een witte hond worstelen op de grond').
% sen_id(10, 9480, 'h', 'TEST', 'yes', 'Twee honden zijn aan het vechten').

